Weak Bursts on Slowly Accreting Neutron Stars

Nearly all observed thermonuclear X-ray bursts are thought to be triggered by the thermally unstable triple-alpha process. Unlike in accreting white dwarfs, the $\gtrsim10^{8} \mathrm{K}$ envelope temperature forces hydrogen burning to proceed via the $\beta$-limited, thermally stable hot CNO cycle. Recent observations of weak X-ray bursts from SAX J1808.4-3658 occurring within 1-3 days of the onset of an accretion outburst have raised the question that these bursts were triggered by thermally unstable hydrogen ignition, analogously to classical novae. Using the stellar evolution code MESA, we explore the unstable ignition of hydrogen on slowly accreting neutron stars. For solar metallicities, the burning is insufficiently vigorous to launch convection and the burst rise is on the envelope thermal timescale, with the hydrogen being consumed over hours. For elevated metallicities ($Z\gtrsim0.06$), however, the initial proton captures onto CNO nuclei heat the envelope enough to drive convection and produce a sharp peak in the luminosity. This peak can match that of the SAX J1808.4-3658 burst, for sufficient enrichment. Following this peak, the hydrogen burning stabilizes at a rate set solely by the ignition depth and CNO abundance in the accreted matter. This quasi-steady-state burning produces an extended tail of elevated emission that lasts until the hydrogen is exhausted. Observations of the tail's luminosity and duration measure the hydrogen and metallicity abundance of the accreted material, while the distance-independent ratio of peak-to-tail luminosities would suggest the presence of significant metallicity gradients prior to convection.

==> st_code.tex <==
% code.tex
% Edward F Brown, Michigan State University
% 
% Macros for commonly used codes
% 
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\flash}{FLASH}
\newcommand{\kepler}{KEPLER}
\newcommand{\nonsmoker}{NON-SMOKER}
\newcommand{\mesa}{\code{MESA}}
\newcommand{\MESA}{\mesa}
\newcommand{\STERN}{STERN}
\newcommand{\ADIPLS}{\code{ADIPLS}}
\newcommand{\DSEP}{DSEP}
\newcommand{\enzo}{\code{ENZO}}
\newcommand{\dStar}{\code{dStar}}
\newcommand{\netJina}{\code{netJina}}
\newcommand{\starType}{\code{starType}}
\newcommand{\AMReX}{\code{AMReX}}
\newcommand{\BoxLib}{\code{BoxLib}}
\newcommand{\Castro}{\code{Castro}}
\newcommand{\Maestro}{\code{Maestro}}
\newcommand{\amrex}{\AMReX}
\newcommand{\boxlib}{\BoxLib}
\newcommand{\castro}{\Castro}
\newcommand{\maestro}{\Maestro}



==> st_derivatives.tex <==
% derivatives.tex
% Edward F Brown, Michigan State University
% 
% typesetting of common derivatives
\ifthenelse{\boolean{@italic_dif}}
{
    \typeout{setting italic derivative symbol}
    \newcommand*{\dif}{\ensuremath{d}}  % differential operator, italic typeface
    \newcommand*{\Dif}{\ensuremath{D}}
}{
    \typeout{setting roman derivative symbol}
    \newcommand*{\dif}{\ensuremath{\mathrm{d}}}  % differential operator, roman typeface
    \newcommand*{\Dif}{\ensuremath{\mathrm{D}}}
}
%derivatives
\newcommand*{\DD}[2]{\mathchoice{\frac{\dif #1}{\dif #2}}{\dif #1/\dif #2}{\dif #1/\dif #2}{\dif #1/\dif #2}} % total derivative
\newcommand*{\dd}[2]{\mathchoice{\frac{\partial #1}{\partial #2}}{\partial#1/\partial#2}{\partial#1/\partial#2}{\partial#1/\partial#2}} % partial derivative
\newcommand*{\jac}[4]{\mathchoice{\frac{\partial(#1,#2)}{\partial(#3,#4)}}{\partial(#1,#2)/\partial(#3,#4)}{\partial(#1,#2)/\partial(#3,#4)}{\partial(#1,#2)/\partial(#3,#4)}} %jacobian
\newcommand*{\tderiv}[3]{\mathchoice{\left(\frac{\partial #1}{\partial #2}\right)_{#3}}{\left(\partial #1/\partial #2\right)_{#3}}{\left(\partial #1/\partial #2\right)_{#3}}{\square}} %thermodynamic derivative

% common shortcuts
\newcommand*{\ddt}[1]{\dd{#1}{t}}    % partial time derivative 
\newcommand*{\DDt}[1]{\DD{#1}{t}}    % total time derivative
\newcommand*{\ddx}[1]{\dd{#1}{x}}    % partial derivative wrt x
\newcommand*{\DDx}[1]{\DD{#1}{x}}    % total derivative wrt x
\newcommand*{\ddy}[1]{\dd{#1}{y}}    % partial derivative wrt y
\newcommand*{\DDy}[1]{\DD{#1}{y}}    % total derivative wrt y
\newcommand*{\ddz}[1]{\dd{#1}{z}}    % partial derivative wrt z
\newcommand*{\DDz}[1]{\DD{#1}{z}}    % total derivative wrt z
\newcommand*{\ddr}[1]{\dd{#1}{r}}    % partial derivative wrt r
\newcommand*{\DDr}[1]{\DD{#1}{r}}    % total derivative wrt r

\ifthenelse{\boolean{@st_vectors}}
{
    \typeout{using boldmath for vectors in fluid derivatives}
    \newcommand*{\derivVec}[1]{\bvec{#1}}
    \newcommand*{\derivGrad}{\grad}
    \newcommand*{\derivDot}{\vdot}
}{
    \typeout{option `vectors' is not selected; falling back on vanilla latex vec command}
    \newcommand*{\derivVec}[1]{\vec{#1}}
    \newcommand*{\derivGrad}{\nabla}
    \newcommand*{\derivDot}{\cdot}
}

\ifthenelse{\boolean{@pound_for_Lie}}                    % Lie derivative
{
    \typeout{using mathsterling for Lie derivative}
    \newcommand*{\LD}[1][]{\ensuremath{\mathsterling_{\derivVec{#1}}}}
}
{
    \typeout{using calligraphic L for Lie derivative}
    \newcommand*{\LD}[1][]{\ensuremath{\mathcal{L}_{\derivVec{#1}}}}
}

% convective derivative and fluid derivative
\newcommand*{\convectiveDerivative}[2][v]{\ddt{#2}+\derivVec{#1}\derivDot\derivGrad #2}
\ifthenelse{\boolean{@uppercase_convective}}
{
    \typeout{setting uppercase D for convective derivative}
    \newcommand*{\convectiveD}[1]{\mathchoice{\frac{\Dif #1}{\Dif t}}{\Dif#1/\Dif#2}{\Dif#1/\Dif#2}{\Dif#1/\Dif#2}}
}{
    \typeout{setting lowercase d for convective derivative}
    \newcommand*{\convectiveD}[1]{\DDt{#1}}
}
\newcommand*{\fluidDerivative}[2][v]{\ddt{#2} + \LD[#1]{#2}}
\newcommand*{\fluidD}[1]{\mathchoice{\frac{\Dif #1}{\Dif t}}{\Dif#1/\Dif t}{\Dif#1/\Dif t}{\Dif#1/\Dif t}}


==> st_instruments.tex <==
% symbols.tex
% Edward Brown, Michigan State University
%
% Observatories, mostly space-based

\newcommand*{\instrument}[1]{{\itshape #1}}
\newcommand*{\rxte}{\instrument{RXTE}}
\newcommand*{\nicer}{\instrument{NICER}}
\newcommand*{\xmm}{\instrument{XMM}}
\newcommand*{\nustar}{\instrument{NuSTAR}}
\newcommand*{\swift}{\instrument{Swift}}
\newcommand*{\xbnews}{\instrument{XB-NEWS}} % according to ADSABS, it is XB-NEWS not XBNEWS
\newcommand*{\chandra}{\instrument{Chandra}}
\newcommand*{\asca}{\instrument{ASCA}}
\newcommand*{\rosat}{\instrument{ROSAT}}
\newcommand*{\einstein}{\instrument{Einstein}}
\newcommand*{\ginga}{\instrument{GINGA}}
\newcommand*{\bbxrt}{\instrument{BBXRT}}
\newcommand*{\suzaku}{\instrument{Suzaku}}
\newcommand*{\bepposax}{\instrument{BeppoSAX}}
\newcommand*{\tess}{\instrument{TESS}}
\newcommand*{\goto}{\instrument{GOTO}}
\newcommand*{\integral}{\instrument{INTEGRAL}}
\newcommand*{\hst}{\instrument{HST}}


==> st_nuclides.tex <==
% nuclides.tex
% Edward F. Brown, Michigan State University
%
% input file with macros for nuclides

% base command
\newcommand*{\nuclei}[2]{\ensuremath{\mathrm{^{#1}#2}}}

% nuclides, with most highest abundance or longest half-life as default
% for example, \carbon produces ^{12}C, \carbon[13] produces ^{13}C
%
\newcommand*{\neutron}{\ensuremath{\mathrm{n}}}
\newcommand*{\nt}{\neutron}
\newcommand*{\proton}{\ensuremath{\mathrm{p}}}
\newcommand*{\pt}{\proton}
\newcommand*{\hydrogen}[1][1]{\nuclei{#1}{H}}
\newcommand*{\helium}[1][4]{\nuclei{#1}{He}}
\newcommand*{\lithium}[1][7]{\nuclei{#1}{Li}}
\newcommand*{\beryllium}[1][9]{\nuclei{#1}{Be}}
\newcommand*{\boron}[1][11]{\nuclei{#1}{B}}
\newcommand*{\carbon}[1][12]{\nuclei{#1}{C}}
\newcommand*{\nitrogen}[1][14]{\nuclei{#1}{N}}
\newcommand*{\oxygen}[1][16]{\nuclei{#1}{O}}
\newcommand*{\fluorine}[1][19]{\nuclei{#1}{F}}
\newcommand*{\neon}[1][20]{\nuclei{#1}{Ne}}
\newcommand*{\sodium}[1][23]{\nuclei{#1}{Na}}
\newcommand*{\magnesium}[1][24]{\nuclei{#1}{Mg}}
\newcommand*{\aluminum}[1][27]{\nuclei{#1}{Al}}
\newcommand*{\silicon}[1][28]{\nuclei{#1}{Si}}
\newcommand*{\phosphorus}[1][31]{\nuclei{#1}{P}}
\newcommand*{\sulfur}[1][32]{\nuclei{#1}{S}}
\newcommand*{\chlorine}[1][35]{\nuclei{#1}{Cl}}
\newcommand*{\argon}[1][36]{\nuclei{#1}{Ar}}
\newcommand*{\potassium}[1][39]{\nuclei{#1}{K}}
\newcommand*{\calcium}[1][40]{\nuclei{#1}{Ca}}
\newcommand*{\scandium}[1][45]{\nuclei{#1}{Sc}}
\newcommand*{\titanium}[1][48]{\nuclei{#1}{Ti}}
\newcommand*{\vanadium}[1][51]{\nuclei{#1}{V}}
\newcommand*{\chromium}[1][52]{\nuclei{#1}{Cr}}
\newcommand*{\manganese}[1][55]{\nuclei{#1}{Mn}}
\newcommand*{\iron}[1][56]{\nuclei{#1}{Fe}}
\newcommand*{\cobalt}[1][59]{\nuclei{#1}{Co}}
\newcommand*{\nickel}[1][58]{\nuclei{#1}{Ni}}
\newcommand*{\copper}[1][63]{\nuclei{#1}{Cu}}
\newcommand*{\zinc}[1][64]{\nuclei{#1}{Zn}}
\newcommand*{\gallium}[1][69]{\nuclei{#1}{Ga}}
\newcommand*{\germanium}[1][74]{\nuclei{#1}{Ge}}
\newcommand*{\arsenic}[1][75]{\nuclei{#1}{As}}
\newcommand*{\selenium}[1][80]{\nuclei{#1}{Se}}
\newcommand*{\bromine}[1][79]{\nuclei{#1}{Br}}
\newcommand*{\krypton}[1][84]{\nuclei{#1}{Kr}}
\newcommand*{\rubidium}[1][85]{\nuclei{#1}{Rb}}
\newcommand*{\strontium}[1][88]{\nuclei{#1}{Sr}}
\newcommand*{\yttrium}[1][89]{\nuclei{#1}{Y}}
\newcommand*{\zirconium}[1][94]{\nuclei{#1}{Zr}}
\newcommand*{\niobium}[1][93]{\nuclei{#1}{Nb}}
\newcommand*{\molybdenum}[1][98]{\nuclei{#1}{Mo}}
\newcommand*{\technetium}[1][97]{\nuclei{#1}{Tc}}
\newcommand*{\ruthenium}[1][102]{\nuclei{#1}{Ru}}
\newcommand*{\rhodium}[1][103]{\nuclei{#1}{Rh }}
\newcommand*{\palladium}[1][106]{\nuclei{#1}{Pd}}
\newcommand*{\silver}[1][107]{\nuclei{#1}{Ag}}
\newcommand*{\cadmium}[1][114]{\nuclei{#1}{Cd}}
\newcommand*{\indium}[1][115]{\nuclei{#1}{In}}
\newcommand*{\tin}[1][120]{\nuclei{#1}{Sn}}
\newcommand*{\antimony}[1][121]{\nuclei{#1}{Sb}}
\newcommand*{\tellurium}[1][130]{\nuclei{#1}{Te}}
\newcommand*{\iodine}[1][127]{\nuclei{#1}{I}}
\newcommand*{\xenon}[1][132]{\nuclei{#1}{Xe}}
\newcommand*{\cesium}[1][133]{\nuclei{#1}{Cs}}
\newcommand*{\barium}[1][138]{\nuclei{#1}{Ba}}
\newcommand*{\lanthanum}[1][139]{\nuclei{#1}{La}}
\newcommand*{\cerium}[1][140]{\nuclei{#1}{Ce}}
\newcommand*{\praseodymium}[1][141]{\nuclei{#1}{Pr}}
\newcommand*{\neodymium}[1][142]{\nuclei{#1}{Nd}}
\newcommand*{\promethium}[1][147]{\nuclei{#1}{Pm}}
\newcommand*{\samarium}[1][152]{\nuclei{#1}{Sm}}
\newcommand*{\europium}[1][153]{\nuclei{#1}{Eu}}
\newcommand*{\gadolinium}[1][158]{\nuclei{#1}{Gd}}
\newcommand*{\terbium}[1][159]{\nuclei{#1}{Tb}}
\newcommand*{\dysprosium}[1][164]{\nuclei{#1}{Dy}}
\newcommand*{\holmium}[1][165]{\nuclei{#1}{Ho}}
\newcommand*{\erbium}[1][168]{\nuclei{#1}{Er}}
\newcommand*{\thulium}[1][169]{\nuclei{#1}{Tm}}
\newcommand*{\ytterbium}[1][174]{\nuclei{#1}{Yb}}
\newcommand*{\lutetium}[1][175]{\nuclei{#1}{Lu}}
\newcommand*{\hafnium}[1][180]{\nuclei{#1}{Hf}}
\newcommand*{\tantalum}[1][180]{\nuclei{#1}{Ta}}
\newcommand*{\tungsten}[1][184]{\nuclei{#1}{W}}
\newcommand*{\rhenium}[1][187]{\nuclei{#1}{Re}}
\newcommand*{\osmium}[1][192]{\nuclei{#1}{Os}}
\newcommand*{\iridium}[1][193]{\nuclei{#1}{Ir}}
\newcommand*{\platnium}[1][195]{\nuclei{#1}{Pt}}
\newcommand*{\gold}[1][197]{\nuclei{#1}{Au}}
\newcommand*{\mercury}[1][202]{\nuclei{#1}{Hg}}
\newcommand*{\thallium}[1][205]{\nuclei{#1}{Tl}}
\newcommand*{\lead}[1][208]{\nuclei{#1}{Pb}}
\newcommand*{\bisumth}[1][209]{\nuclei{#1}{Bi}}
\newcommand*{\polonium}[1][210]{\nuclei{#1}{Po}}
\newcommand*{\astatine}[1][210]{\nuclei{#1}{At}}
\newcommand*{\radon}[1][222]{\nuclei{#1}{Rn}}
\newcommand*{\francium}[1][223]{\nuclei{#1}{Fr}}
\newcommand*{\radium}[1][226]{\nuclei{#1}{Ra}}
\newcommand*{\actinium}[1][227]{\nuclei{#1}{Ac}}
\newcommand*{\thorium}[1][232]{\nuclei{#1}{Th}}
\newcommand*{\protactinium}[1][231]{\nuclei{#1}{Pa}}
\newcommand*{\uranium}[1][238]{\nuclei{#1}{U}}
\newcommand*{\neptunium}[1][237]{\nuclei{#1}{Np}}
\newcommand*{\plutonium}[1][244]{\nuclei{#1}{Pu}}
\newcommand*{\americium}[1][243]{\nuclei{#1}{Am}}
\newcommand*{\curium}[1][247]{\nuclei{#1}{Cm}}
\newcommand*{\berkelium}[1][247]{\nuclei{#1}{Bk}}
\newcommand*{\californium}[1][251]{\nuclei{#1}{Cf}}
\newcommand*{\einsteinium}[1][252]{\nuclei{#1}{Es}}
\newcommand*{\fermium}[1][257]{\nuclei{#1}{Fm}}
\newcommand*{\mendelevium}[1][258]{\nuclei{#1}{Md}}
\newcommand*{\nobelium}[1][259]{\nuclei{#1}{No}}
\newcommand*{\lawrencium}[1][262]{\nuclei{#1}{Lr}}
\newcommand*{\rutherfordium}[1][261]{\nuclei{#1}{Rf}}
\newcommand*{\dubnium}[1][268]{\nuclei{#1}{Db}}
\newcommand*{\seaborgium}[1][271]{\nuclei{#1}{Sg}}
\newcommand*{\bohrium}[1][274]{\nuclei{#1}{Bh}}
\newcommand*{\hassium}[1][270]{\nuclei{#1}{Hs}}
\newcommand*{\meitnerium}[1][278]{\nuclei{#1}{Mt}}
\newcommand*{\darmstadtium}[1][281]{\nuclei{#1}{Ds}}
\newcommand*{\roentgenium}[1][281]{\nuclei{#1}{Rg}}
\newcommand*{\copernicum}[1][285]{\nuclei{#1}{Cn}}


==> st_symbols.tex <==
% symbols.tex
% Edward Brown, Michigan State University
%
% symbols for commonly used expressions in stellar astrophysics.


\newcommand*{\epsnuc}{\ensuremath{\epsilon_{\mathrm{nuc}}}}	% nuclear heating rate
\newcommand*{\epsgrav}{\ensuremath{\epsilon_{\mathrm{grav}}}} % gravitational heating rate
\newcommand*{\epsnu}{\ensuremath{\epsilon_{\mathrm{\nu}}}} % neutrino losses
\newcommand*{\Teff}{\ensuremath{T_{\!\mathrm{eff}}}}	% effective temperature
\newcommand*{\teff}{\Teff}
\newcommand*{\Ledd}{\ensuremath{L_{\mathrm{Edd}}}} % Eddington Luminosity
\newcommand*{\logg}{\ensuremath{\log g}}	% log surface gravity
\newcommand*{\Tc}{\ensuremath{T_{\mathrm{\!c}}}} % central temperature
\newcommand*{\Pc}{\ensuremath{P_{\mathrm{\!c}}}} % central pressure
\newcommand*{\rhoc}{\ensuremath{\rho_{\mathrm{c}}}} % central density
\newcommand*{\CP}{\ensuremath{C_{\!P}}} % specific heat at constant pressure
\newcommand*{\Mdot}{\ensuremath{\dot{M}}} % mass-loss rate

% for correction between baryon densities and mass-energy densities
\newcommand*{\nB}{\ensuremath{n_{\mathrm{B}}}}	% baryon density

% thermodynamical Gammas
\newcommand*{\Gammaone}{\ensuremath{\Gamma_{\!1}}} % $ (\partial\ln P/\partial \ln\rho)_S$
\newcommand*{\Gammatwo}{\ensuremath{\Gamma_{\!2}}} % $ \left[1-(\partial\ln T/\partial\ln P)_S\right]^{-1}$
\newcommand*{\Gammathree}{\ensuremath{\Gamma_{\!3}}} % $ 1+ (\partial\ln T/\partial\ln\rho)_S$

% stellar gradients
\newcommand*{\alphaMLT}{\ensuremath{\alpha_{\mathrm{MLT}}}}	% mixing length parameter
\newcommand*{\chirho}{\ensuremath{\chi_{\rho}}}	% $(\partial\ln P/\partial\ln\rho)_T$
\newcommand*{\chiT}{\ensuremath{\chi_{\raisebox{-2pt}{$\scriptstyle T$}}}}	% $(\partial\ln P/\partial\ln T)_{\rho}$
\newcommand*{\Dov}{\ensuremath{D_{\mathrm{ov}}}}	% overshoot diffusion coefficient
\newcommand*{\nablaad}{\ensuremath{\nabla_{\!\mathrm{ad}}}}	% adiabatic temperature gradient
\newcommand*{\nablarad}{\ensuremath{\nabla_{\!\mathrm{rad}}}}	% radiative temperature gradient
\newcommand*{\nablaT}{\ensuremath{\nabla_{\!T}}}	% actual temperature gradient
\newcommand*{\nablaL}{\ensuremath{\nabla_{\mathrm{\!L}}}}	% Ledoux criterion
\newcommand*{\scaleheight}{\ensuremath{\lambda_P}}	% pressure scale height
\newcommand*{\Pgas}{\ensuremath{P_{\!\!\mathrm{gas}}}}	% gas pressure

% more symbols for radiation and gas pressures
\newcommand*{\Prad}{\ensuremath{P_{\!\!\mathrm{rad}}}}	% radiation pressure
\newcommand*{\Lrad}{\ensuremath{L_{\mathrm{rad}}}}	% radiative luminosity
\newcommand*{\Fconv}{\ensuremath{F_{\!\mathrm{conv}}}}		% convective flux
\newcommand*{\Frad}{\ensuremath{F_{\!\mathrm{rad}}}}	% radiative flux

% mixing symbols
\newcommand*{\alphasc}{\ensuremath{\alpha_{\mathrm{sc}}}} % semiconvection efficiency parameter
\newcommand*{\alphath}{\ensuremath{\alpha_{\mathrm{th}}}} % thermohaline efficiency parameter
\newcommand*{\Dth}{\ensuremath{D_{\mathrm{th}}}} % thermohaline diffusion coefficient
\newcommand*{\fov}{\ensuremath{f_{\mathrm{ov}}}} % convective overshoot parameter

% physical constants
\newcommand*{\kB}{\ensuremath{k_\mathrm{B}}} % Boltzmann constant
\newcommand*{\NA}{\ensuremath{N_\mathrm{\!A}}} % Avogadro number
\newcommand*{\mb}{\ensuremath{m_\mathrm{u}}} % atomic mass unit
\newcommand*{\sigmaSB}{\ensuremath{\sigma_\mathrm{\!SB}}} % Stefan-Boltzmann constant
\newcommand*{\pF}{\ensuremath{p_\mathrm{F}}} %Fermi momentum
\newcommand*{\EF}{\ensuremath{E_\mathrm{F}}} %Fermi energy
\newcommand*{\me}{\ensuremath{m_\mathrm{e}}} %electron mass
\newcommand*{\mpr}{\ensuremath{m_\mathrm{p}}} %proton mass
\newcommand*{\mn}{\ensuremath{m_\mathrm{n}}} %neutron mass
\newcommand*{\alphaF}{\ensuremath{\alpha}} %Fine structure
\newcommand*{\lambdaD}{\ensuremath{\lambda_{\mathrm{D}}}} %Debye length
\newcommand*{\abohr}{\ensuremath{a_{\mathrm{B}}}} %Bohr radius


% stellar parameters
\newcommand*{\tkh}{\ensuremath{\tau_{\mathrm{KH}}}} % thermal (Kelvin-Helmholtz) timescale

% asteroseismology
\newcommand*{\cs}{\ensuremath{c_{\rm s}}} % adiabatic sound speed
\newcommand*{\Slamb}{\ensuremath{S_{\!\ell}}} % Lamb frequency

% fluids, dimensionless numbers
\newcommand*{\fluidnumber}[1]{\ensuremath{\mathrm{#1}}}
\newcommand*{\Ma}{\fluidnumber{Ma}}	% Mach number
\newcommand*{\Rey}{\fluidnumber{Re}}	% Reynolds number
\newcommand*{\Da}{\fluidnumber{Da}} % Damk\"ohler number
\newcommand*{\lG}{\ensuremath{\ell_{\mathrm{G}}}} % Gibson length



==> st_units.tex <==
% units.tex
% Edward F Brown, Michigan State University
% 
% typesetting of dimensional values
% Features: proper spacing between value and unit; unit is set in correct type

% powers
\newcommand*{\ee}[1]{\ensuremath{\times 10^{#1}}}		% 3.0\ee{4} => 3.0\times 10^{4}
\newcommand*{\sci}[2]{\ensuremath{#1\ee{#2}}}			% \sci{3.0}{4} => 3.0\times 10^{4}
\newcommand{\power}[2]{\ensuremath{{#1}^{#2}}}		    % \power{2}{3} => 2^{3}

% per APS style, there is a full space between value and unit, and a thin space between unit components
\newcommand*{\valueskip}{\;}
\newcommand*{\vsk}{\valueskip}
\newcommand*{\unitskip}{\,}
\newcommand*{\usk}{\unitskip}
\newcommand*{\val}[2]{\ensuremath{#1\valueskip#2}}

% sometimes you want to input a range of numbers
% example: \rng{2}{3} puts 2 to 3; \rng[--]{2}{3} puts 2--3, where the two dashes are correctly typeset 
% as an en-dash rather than as a minus sign
\newcommand*{\rng}[3][~to~]{\ensuremath{#2\textrm{#1}#3}}
% this puts in a range with a unit
% example: \valrng[--]{2}{3}{\times \val{10^{3}}{\kilo\gram}}
\newcommand*{\valrng}[4][~to~]{\ensuremath{\left(#2\textrm{#1}#3\right)#4}}


% units should be in upright (roman) font
\newcommand*{\unitstyle}[1]{\mathrm{#1}}

% pre-defined macros for common units
% prefixes
\newcommand*{\yocto}{\unitstyle{y}}		% 10^{-24}
\newcommand*{\zepto}{\unitstyle{z}}		% 10^{-21}
\newcommand*{\atto}{\unitstyle{a}}		% 10^{-18}
\newcommand*{\femto}{\unitstyle{f}}		% 10^{-15}
\newcommand*{\pico}{\unitstyle{p}}		% 10^{-12}
\newcommand*{\nano}{\unitstyle{n}}		% 10^{-9}
\newcommand*{\micro}{\unitstyle{\mu}}	% 10^{-6}
\newcommand*{\milli}{\unitstyle{m}}		% 10^{-3}
\newcommand*{\centi}{\unitstyle{c}}		% 10^{-2}
\newcommand*{\deci}{\unitstyle{d}}		% 10^{-1}
%
\newcommand*{\deka}{\unitstyle{da}}		% 10^{1}
\newcommand*{\hecto}{\unitstyle{h}}		% 10^{2}
\newcommand*{\kilo}{\unitstyle{k}}		% 10^{3}
\newcommand*{\Mega}{\unitstyle{M}}		% 10^{6}
\newcommand*{\Giga}{\unitstyle{G}}		% 10^{9}
\newcommand*{\Tera}{\unitstyle{T}}		% 10^{12}
\newcommand*{\Peta}{\unitstyle{P}}		% 10^{15}
\newcommand*{\Exa}{\unitstyle{E}}		% 10^{18}
\newcommand*{\Zetta}{\unitstyle{Z}}		% 10^{21}
\newcommand*{\Yotta}{\unitstyle{Y}}		% 10^{24}

% base units, mks
\newcommand*{\meter}{\unitstyle{m}}     % SI length
\newcommand*{\kilogram}{\kilo\gram}     % SI mass
\newcommand*{\second}{\unitstyle{s}}    % SI time

\newcommand*{\Kelvin}{\unitstyle{K}}
\newcommand*{\K}{\Kelvin}  %degrees Kelvin

% base units, cgs
\newcommand*{\cm}{\centi\meter}         % cgs length
\newcommand*{\gram}{\unitstyle{g}}      % cgs mass

% derived units
\newcommand*{\grampercc}{\gram\unitskip\power{\cm}{-3}} % mass density
\newcommand*{\grampersquarecm}{\gram\unitskip\power{\cm}{-2}} % column depth
\newcommand*{\GramPerCc}{\grampercc}
\newcommand*{\GramPerSc}{\grampersquarecm}
\newcommand*{\columnunit}{\grampersquarecm}     % mass column density
\newcommand*{\dyne}{\unitstyle{dyn}}            % dyne
\newcommand*{\erg}{\unitstyle{erg}}             % ergs
\newcommand*{\ergs}{\erg}
\newcommand*{\gauss}{\unitstyle{G}}             % gauss
\newcommand*{\ergspersecond}{\erg\unitskip\power{\second}{-1}}  % luminosity
\newcommand*{\ergspergram}{\erg\unitskip\power{\gram}{-1}}  % energy per mass
\newcommand*{\cgsflux}{\erg\unitskip\power{\cm}{-2}\unitskip\power{\second}{-1}} % flux

% Nuclear and atomic units
\newcommand*{\amu}{\unitstyle{u}}               %atomic mass unit
\newcommand*{\angstrom}{\mbox{\AA}}             %Angstrom
\newcommand*{\fermi}{\femto\meter}              %fermi
\newcommand*{\eV}{\unitstyle{eV}}               %eV
\newcommand*{\keV}{\kilo\eV}                    %keV
\newcommand*{\MeV}{\Mega\eV}                    %MeV
\newcommand*{\GeV}{\Giga\eV}                    %GeV
% Beam units
\newcommand*{\MeVA}{\MeV/A}                     % MeV per nucleon
\newcommand*{\GeVA}{\GeV/A}                     % GeV per nucleon

% solar and astronomical units
\newcommand*{\Msun}{\ensuremath{M_\odot}}       % solar mass
\newcommand*{\Lsun}{\ensuremath{L_\odot}}       % solar luminosity
\newcommand*{\Rsun}{\ensuremath{R_\odot}}       % solar radius
\newcommand*{\yr}{\unitstyle{yr}}               % Calendar year, 365 d
\newcommand*{\julyr}{\unitstyle{a}}             % Julian year = 365.25 * 86400 s
\newcommand*{\Myr}{\Mega\yr}                    % $10^{6}\,\yr$
\newcommand*{\Gyr}{\Giga\yr}                    % $10^{9}\,\yr$
\newcommand*{\AU}{\unitstyle{au}}               % astronomical unit
\newcommand*{\parsec}{\unitstyle{pc}}           % parsec
\newcommand*{\kpc}{\kilo\parsec}                % kiloparsec
\newcommand*{\Jansky}{\unitstyle{Jy}}           % Jansky
\newcommand*{\mJy}{\unitstyle{\mu Jy}}          % micro Jansky
\newcommand*{\Msunperyr}{\Msun\unitskip\power{\yr}{-1}}	% solar masses per year

% misc. units
\newcommand*{\minute}{\unitstyle{m}}            % minute = 60 s
\newcommand*{\hour}{\unitstyle{h}}              % hour = 60 * 60 s
\newcommand*{\aday}{\unitstyle{d}}              % IAU definition: d = 86400 s (\day aleady in use)
\newcommand*{\km}{\kilo\meter}                  % kilometers
\newcommand*{\Hz}{\unitstyle{Hz}}               % Hertz
\newcommand*{\ksec}{\kilo\second}               % kilosecond
\newcommand*{\mol}{\unitstyle{mol}}             % mole
\newcommand*{\barn}{\ensuremath{\mathrm{b}}}    % 10**-24 cm**2 = 100 fm**2
\newcommand*{\Crab}{\unitstyle{Crab}}           % this one is hard to describe
\newcommand*{\mCrab}{\milli\Crab}


==> st_vectors.tex <==
% vectors.tex
% Edward Brown, Michigan State University
%
% Some basic vector operators
%
% Requires package bm.sty
%

\RequirePackage{bm}
\newcommand{\bvec}[1]{\ensuremath{\bm{#1}}} % boldface vector style
\newcommand{\grad}{\bvec{\nabla}} % gradient
\newcommand{\divr}{\nabla \cdot} % divergence
\newcommand{\curl}{\bvec{\nabla \times}} % curl
\newcommand{\lap}{\ensuremath{\nabla^2}} % Laplacian
\newcommand{\btens}[1]{\ensuremath{\bm{\mathsf{#1}}}}   % tensor
\newcommand{\vcross}{\bvec{\times}} % cross product
\newcommand{\vdot}{\bvec{\cdot}} % dot product

